Automatic Short Answer Grading via Multiway Attention Networks

Automatic short answer grading (ASAG), which autonomously score student answers according to reference answers, provides a cost-effective and consistent approach to teaching professionals and can reduce their monotonous and tedious grading workloads. However, ASAG is a very challenging task due to two reasons: (1) student answers are made up of free text which requires a deep semantic understanding; and (2) the questions are usually open-ended and across many domains in K-12 scenarios. In this paper, we propose a generalized end-to-end ASAG learning framework which aims to (1) autonomously extract linguistic information from both student and reference answers; and (2) accurately model the semantic relations between free-text student and reference answers in open-ended domain. The proposed ASAG model is evaluated on a large real-world K-12 dataset and can outperform the state-of-the-art baselines in terms of various evaluation metrics.

==> implementation.tex <==
We use 64-dimensional pre-trained word embeddings which are jointly learning during training, and zero vectors for out-of-vocabulary words. We stack 2 bidirectional transformer block in both transformer layer and inside layer, and in each block, we employ 4 attention heads. We apply dropout between layers, with dropout rate 0.1, and AdaDelta optimization method with initial learning rate 1.0.


==> notation.tex <==
\begin{table}[t]
\centering
\caption{Symbols.}
\label{tab:symbols}
\begin{tabular}{l|l}
\toprule
\textbf{Symbol} & \textbf{Definition and Description} \\ \midrule

$transformer(\cdot)$ & the transformer encoding unit \\
$softmax(\cdot)$ & the standard softmax function \\
$(\cdot)^\top$ & matrix transpose \\ 
$\odot$ & dot product \\ 
$d$ & the dimension of the hidden states \\
$n$ & the number of words in student/reference answers \\
\midrule

$\mathbf{w}_i^q$, $\mathbf{w}_i^p$ & the \emph{i}th word in student, reference answer \\
$\mathbf{h}_i^q$, $\mathbf{h}_i^p$ & the hidden state vector of $\mathbf{w}_i^q$, $\mathbf{w}_i^p$ after transformer encoding unit \\
$\mathbf{s}_i^q$, $\mathbf{s}_i^p$ & the self-attentive representations of $\mathbf{h}_i^q$, $\mathbf{h}_i^p$ after self-attention unit \\
$\mathbf{o}_i^q$, $\mathbf{o}_i^p$ & the aggregation of transformer hidden states and self-attentive \\
& representations, i.e., $\mathbf{o}_i^p = [\mathbf{h}_i^q, \mathbf{s}_i^q]$ and $\mathbf{o}_i^q = [\mathbf{h}_i^p, \mathbf{s}_i^p]$ \\
\midrule

$(\cdot)^a$, $(\cdot)^s$, $(\cdot)^m$, $(\cdot)^d$ & the superscripts representing additive, subtractive, multiplicative \\
& and dot-product attention functions \\
$\Theta^a$, $\Theta^s$, $\Theta^m$, $\Theta^d$ & the parameters in additive, subtractive, multiplicative \\
& and dot-product attention functions \\
$\mathbf{h}_i^a$, $\mathbf{h}_i^s$, $\mathbf{h}_i^m$, $\mathbf{h}_i^d$ & the representations weighted by additive, subtractive, multiplicative \\ 
& and dot-product attention scores \\
$e^{(\cdot)}_{(\cdot)}$, $\alpha^{(\cdot)}_{(\cdot)}$ & the raw and normalized attention scores from different functions \\ 
& at different positions \\ 
$\mathbf{t}_i^w$ & the aggregation of matching information, i.e., $\mathbf{t}_i^w = [\mathbf{h}_i^a, \mathbf{h}_i^s, \mathbf{h}_i^m, \mathbf{h}_i^d]$ \\
\midrule

$\mathbf{H}^q$, $\mathbf{H}^p$, $\mathbf{H}^w$ & the linear mapping matrices \\
$\mathbf{g}_i^q$, $\mathbf{g}_i^p$, $\mathbf{h}_i^w$ & the representations after linear mapping, i.e., $\mathbf{g}_i^q = \mathbf{H}^q \mathbf{o}_i^q$, \\
& $\mathbf{g}_i^p = \mathbf{H}^p \mathbf{o}_i^p$, and $\mathbf{h}_i^w = \mathbf{H}^w \mathbf{t}_i^w$ \\ 
$\mathbf{z}_i$ & the smooth representation after transformer aggregation, \\
& i.e., $\mathbf{z}_i = transformer([\mathbf{g}_i^q, \mathbf{g}_i^p, \mathbf{h}_i^w])$ \\
$\mathbf{Z}$ & the concatenation of $\mathbf{z}_i$s \\
\bottomrule
\end{tabular}
\vspace{-0.7cm}
\end{table}


==> related.tex <==
Various ASAG approaches have been studied by both educational machine learning and natural language processing communities over the past years. In general, approaches of ASAG can be divided into four categories. The first one is pattern learning approaches which pull out pertinent information from a partially syntactically analyzed text by applying a set of domain specific patterns typically built from training data~\cite{sukkarieh2003auto,sukkarieh2004auto,moodle2019,leacock2003c,mitchell2002towards,ramachandran2015identifying,makatchev2007combining}. The grading is based the matches which indicate that a question has been answered correctly. The second category involves hand-crafted feature based models that extract various linguistic features from both reference answers and student answers and apply existing machine learning algorithms to make the final scoring and grading~\cite{mohler2009text,mohler2011learning,ott2013comet,Yannakoudakis2011AND}. The third types are embedding based models which learn embedding networks from either general or educational specific corpus~\cite{mikolov2013distributed,pennington2014glove,Conneau2017SupervisedLO}. The last category includes end-to-End Deep Models. Different from embedding based models, approaches in end-to-end deep learning models aim to solve the grading problem directly by training the deep supervised network with existing scoring~\cite{Alikaniotis2016Automatic,Kumar2017,antipov2015learned,tran2015learning,feng2018language}.
%In the end-to-end deep model training, the goal of accurate grading is directly optimized compared to embedding based approaches that learn the universal representations 

% \begin{itemize}
% \item Pattern learning that manually or automatically extract scoring patterns by using the classic information extraction techniques (Section \ref{sec:pattern}).
% \item Hand-crafted feature based approaches that rely on mature ML tools (i.e., dependency parsers, part-of-speech taggers, etc.) to extract pre-defined linguistic features. The predictions are made by either supervised or unsupervised ML models with these hard-crafted features (Section \ref{sec:hand}).
% \item Embedding based approaches which learn word level or sentence level embedding networks  followed by training a classifier (Section \ref{sec:embedding}).
% \item End-to-end deep models that directly captures the semantic relationship between student answers and the reference answer (Section \ref{sec:deep}).
% \end{itemize}

% \vspace{-0.3cm}
% \subsection{Pattern Learning}
% \label{sec:pattern}
% \vspace{-0.2cm}

% Pattern learning based approaches pull out pertinent information from a partially syntactically analyzed text by applying a set of domain specific patterns typically built from training data \cite{sukkarieh2003auto,sukkarieh2004auto,moodle2019}. The grading is based the matches which indicate that a question has been answered correctly. In general, there are two ways to generate these patterns: (1) manually-engineered patterns; and (2) automatic learned patterns. In the manual pattern based approaches, specific domain knowledge is required to determine all the ways in which the reference answer is expressed by different students and think of all the plausible variances of student answers. For examples, Bachman et al. extracted regular expressions from reference answers to generate the scoring keys \cite{bachman2002reliable}. Makatchev and VanLehn encoded first-order predicate representations of reference answers to score student responses \cite{makatchev2007combining}. While in the automatic pattern learning, the patterns are automatically learned from annotated corpus by using keywords, synonyms, and n-grams \cite{leacock2003c,mitchell2002towards}. Rramachandran et al. used word-order graphs to identify important patterns from both reference answers and top-scoring student answers. They extracted both content tokens and phrases for measuring the semantic relatedness \cite{ramachandran2015identifying}. 

% \vspace{-0.3cm}
% \subsection{Hand-crafted Feature based Models}
% \label{sec:hand}
% \vspace{-0.2cm}

% Hand-crafted feature based models usually extract various linguistic features from both reference answers and student answers. These features contains both syntactic and semantic information. Both supervised and unsupervised learning algorithms are applied to make the final scoring and grading \cite{mohler2009text,mohler2011learning,ott2013comet,Yannakoudakis2011AND}. For examples, Mohler and Mihalcea used a number of knowledge-based and corpus-based text similarity functions to automatically assign a grade to a student answer by comparing with similar answers with grading scores \cite{mohler2009text}. Ott et al. learned a meta-classifier by combining three different grade prediction systems, which are build on linguistic features from reference and student answers \cite{ott2013comet}.  Mohler et al. combined several graph alignment features and aligned the dependency graph of the reference and student answers in order to make use of a structural component in the ASAG task \cite{mohler2011learning}. Farra et al. used logistic regression to score persuasive essays based on opinion and topic related features \cite{Farra2015ScoringPE}. 

% \vspace{-0.3cm}
% \subsection{Embedding based Models}
% \label{sec:embedding}
% \vspace{-0.2cm}

% Embedding based models learn embedding networks from either general or educational specific corpus. These embedding networks will be used to extract and abstract context-aware semantic information at different levels. In text mining and natural language understanding, words, phrases, sentences are represented as embeddings to solve many real-world tasks \cite{mikolov2013distributed,pennington2014glove}. Saha et al. demonstrated the benefits of using both word and sentence level embeddings for ASAG tasks especially for out-of-domain and non-sentential answers \cite{Saha2018}. Conneau et al. proposed to train universal sentence representations by using the supervised data of the Stanford Natural Language Inference datasets. The representation is learned by using the bidirectional long short-term memory (LSTM) network \cite{Conneau2017SupervisedLO}.

% \vspace{-0.3cm}
% \subsection{End-to-End Deep Models}
% \label{sec:deep}
% \vspace{-0.2cm}

% Different from embedding based models, approaches in end-to-end deep learning models aim to solve the grading problem directly by training the deep supervised network with existing scoring. In the end-to-end deep model training, the goal of accurate grading is directly optimized compared to embedding based approaches that learn the universal representations \cite{Alikaniotis2016Automatic,Kumar2017}. Alikaniotis et tal. applied LSTMs to represent the meaning of texts by training the recurrent neural network with known grading scores \cite{Alikaniotis2016Automatic}. Kumar et al. developed a cascaded framework for ASAG by stacking Siamese bidirectional LSTM layers, an earth-mover distance pooling layer, and a support vector ordinal regression output layer \cite{Kumar2017}. The proposed approach in this paper belongs to this category. An effective and efficient end-to-end model is built to accurately model the semantic relations between free-text student answers and reference answers.

% However, most of the current approaches proposed to solve this problem are based on hand-crafted features that are manually designed to encode the structural and semantic information in texts \cite{mitchell2002towards, nielsen2009recognizing,ramachandran2015identifying}. Thus, the performance of such approaches could be largely constrained by human's feature engineering ability, which could be ineffective in capturing sufficient information \cite{antipov2015learned,tran2015learning,feng2018language}. In addition, the rules to generate hand-craft features from text in one domain could have very limited generalization ability and can not work effectively in other domains. Thus, dedicated efforts are desired to develop more advanced models that are able to automatically understand reference and student answers and accurately capture their relations. 

